Coherence in Molecular Photoionization

The development of attosecond technology has enabled the real-time observation of coherent electron motion in atoms, molecules and condensed phases. Experimentally, it is now possible to generate laser pulses of durations of only a few tens of attoseconds. These durations are of the order of the revolution period of the first Bohr orbit (150 asec), opening the way to visualize and even control electron dynamics at its natural time scale. This PhD thesis constitutes a theoretical study of fundamental phenomena occurring in gas-phase molecules upon interaction with light. We have investigated ultrafast charge migration in biological molecules initiated by attosecond XUV pulses. In addition, we have studied the high-energy interferences that arise in the vibrationally-resolved photoelectron spectra of small polyatomic molecules. In order to explore these complex phenomena, we have employed numerical methods that describe molecular photoionization by evaluating continuum scattering wave functions, allowing us to compute different observables such as time-dependent electron densities or photoionization cross sections.

==> Chapters/Resumen-initialVersion.tex <==
\chapter*{Resumen}
\label{Resumen}
% \addcontentsline{toc}{part}{Resumen}
\fancyhead[LE]{}
\fancyhead[RO]{\fontsize{11pt}{11pt}\selectfont Resumen}

Presentamos un estudio te\'orico de procesos inducidos por luz en mol\'eculas en fase gaseosa, analizando procesos f\'isicos que surgen en dos contextos diferentes: utilizando radiaci\'on sincrotr\'on y pulsos l\'aser ultra-cortos.
Este trabajo ha sido realizado en estrecha colaboraci\'on con Piero Decleva (Universit\`a degli Studi di Trieste).\vspace{2 mm}

En primer lugar, presentamos un estudio sobre fotoionizaci\'on de capa interna de mol\'eculas diat\'omicas (CO) y poliat\'omicas (CF$_4$, BF$_3$) a altas energ\'ias de fotoelectr\'on que ha sido realizado en colaboraci\'on con los grupos experimentales de Edwin Kukk (Turku University), Catalin Miron (Synchrotron SOLEIL), Kiyosi Ueda (Synchrotron SPring-8) y Thomas Darrah Thomas (Oregon State University).
La combinaci\'on de c\'alculos avanzados basados en la Teor\'ia del Funcional de la Densidad (DFT, del ingl\'es ``Density Functional Theory''), capaces de describir procesos de fotoionizaci\'on teniendo en cuenta los grados de libertad nucleares, junto con el uso de instalaciones sincrotr\'on de tercera generaci\'on, ha permitido la investigaci\'on de desviaciones de la aproximaci\'on de Franck-Condon, observables en espectros fotoelectr\'onicos resueltos vibracionalmente.
Demostramos que la respuesta nuclear a la difracci\'on electr\'onica es observable y que, por lo tanto, puede utilizarse para obtener informaci\'on estructural.
Como prueba de concepto, utilizando c\'alculos DFT como herramienta de an\'alisis para el ajuste de datos experimentales, hemos determinado con precisi\'on la distancia de equilibrio de la mol\'ecula de CO y la contracci\'on de enlace que tiene lugar tras la extracci\'on de un electr\'on del orbital 1s del \'atomo de carbono.
Esto representa una ventaja de la espectroscop\'ia fotoelectr\'onica con respecto a t\'ecnicas espectrosc\'opicas m\'as convencionales, que, en general, tan solo proporcionan informaci\'on estructural de la especie neutra.
Adem\'as, hemos analizado un fen\'omeno distinto que tiene lugar cuando se emite un electr\'on desde un orbital deslocalizado: emisi\'on multic\'entrica.
Los resultados obtenidos para la mol\'ecula de fl\'uor mediante simulaciones num\'ericas est\'an de acuerdo, de forma cualitativa, con los proporcionados por la sencilla f\'ormula propuesta por Cohen y Fano en los a\~nos sesenta.\vspace{2 mm}

Hemos empleado la misma metodolog\'ia basada en DFT junto con teor\'ia de perturbaciones a primer orden y un formalismo de matriz de densidad reducida para reportar la primera observaci\'on experimental de din\'amica electr\'onica en una mol\'ecula biol\'ogica: el amino \'acido fenilalanina, en colaboraci\'on con los grupos experimentales de Mauro Nisoli (Politecnico di Milano), Luca Poletto (Istituto Nazionale di Fotonica - Consiglio Nazionale delle Ricerche) y Jason Greenwood (Queen's University).
El uso de pulsos de attosegundos, en combinaci\'on con novedosas t\'ecnicas de detecci\'on, ha permitido la captura de din\'amica puramente electr\'onica en su escala de tiempo natural.
Debido a sus anchos espectros energ\'eticos, los pulsos de attosegundos son herramientas ideales para generar superposiciones coherentes de estados, induciendo una respuesta electr\'onica ultra-r\'apida que puede ser visualizada con resoluci\'on de attosegundos.
Nuestro estudio te\'orico ha permitido interpretar los hallazgos experimentales en t\'erminos de migraci\'on de carga, confirmando la primera observaci\'on de din\'amica puramente electr\'onica en una biomol\'ecula.
Hemos extendido este trabajo al estudio de los amino \'acidos glicina y tript\'ofano, lo cual ha permitido la investigaci\'on de efectos debidos a la sustituci\'on del radical en el mecanismo de la migraci\'on de carga.


==> Chapters/blank.tex <==
        \newpage
        \phantom{placeholder} % doesn't appear on page
        \thispagestyle{empty} % if want no header/footer
        \newpage
